Preserving Tumor Volumes for Unsupervised Medical Image Registration

Medical image registration is a critical task that estimates the spatial correspondence between pairs of images. However, current traditional and deep-learning-based methods rely on similarity measures to generate a deforming field, which often results in disproportionate volume changes in dissimilar regions, especially in tumor regions. These changes can significantly alter the tumor size and underlying anatomy, which limits the practical use of image registration in clinical diagnosis. To address this issue, we have formulated image registration with tumors as a constraint problem that preserves tumor volumes while maximizing image similarity in other normal regions. Our proposed strategy involves a two-stage process. In the first stage, we use similarity-based registration to identify potential tumor regions by their volume change, generating a soft tumor mask accordingly. In the second stage, we propose a volume-preserving registration with a novel adaptive volume-preserving loss that penalizes the change in size adaptively based on the masks calculated from the previous stage. Our approach balances image similarity and volume preservation in different regions, i.e., normal and tumor regions, by using soft tumor masks to adjust the imposition of volume-preserving loss on each one. This ensures that the tumor volume is preserved during the registration process. We have evaluated our strategy on various datasets and network architectures, demonstrating that our method successfully preserves the tumor volume while achieving comparable registration results with state-of-the-art methods. Our codes is available at: \url{https://dddraxxx.github.io/Volume-Preserving-Registration/}.

==> iccv2023AuthorKit/rebuttal/metrics.tex <==
\textbf{Validity of STSR (\Ro \&\Rth)}
Since our goal is to preserve tumor volumes while maximizing image similarity in other normal regions, we use evaluation metrics to measure these two objectives separately. We adopt Dice and landmark distances to measure registration error, but it is important to note that they only measure the accuracy of normal regions that will not be affected by tumor. Specifically, Dice primarily focuses on aligning the outline of the foreground, disregarding the registration of inner content. The landmarks selected for evaluation are located away from tumors because tumor growth can extrude surrounding tissues, making landmarks around it unreliable. Therefore, our improvement in Dice and landmark is minor as pointed by \Ro, and these metrics are only used to show comparable accuracy in non-tumor regions (as claimed in Line 724-729, 738-740). 

The advantage of our method lies in tumor volume preservation. However, this objective has been barely considered by previous registration methods, and there is no existing metric to evaluate it. To bridge this gap, we must introduce STSR as an innovative approach that offers a direct measurement of tumor changes during registration, surpassing limitations of other common metrics like Dice and Landmark Distance in tumor regions. We also want to emphasize that there is no bias in evaluating with STSR (\Rth), as our method does not explicitly optimize STSR. STSR calculation requires tumor and organ GT segmentations, which are unknown in our optimization. Additionally, two other widely-used metrics defined on the Jacobian matrix, which measures the amount of foldovers (($|J_\theta|<0(\%)$) and distorted volumes (Std. $|J_\theta|$) in the registration flow, also validates the effectiveness of our volume preservation.

%{ why STSR? -- 1. few similar works 2.motivation and other could not.
%Tumor volume-preserving registration is crucial in clinical applications, yet there is a shortage of recent works on this topic. To bridge this gap, we introduce STSR and TSR as innovative approaches that tackle the scarcity of volume-preservation metrics in evaluations.
% Volume-preserving registration for tumors is an important topic in clinical application while we found there is relatively few recent works discussing it. Therefore, we utilize STSR and TSR to address the lack of metrics in terms of volume-preservation in evaluation. 

% STSR can directly measure the change of tumors during registration while other common metrics, such as Dice and Landmark Distance, failed to do so. Dice score only indicate how well the outline of the foreground is aligned. Since the tumor lies inside the organ, the tumor information is not included in the outline, and thus not in the Dice sore. As of Landmark Distance, it is noted the position of landmarks near tumor area will be affected by the growth of tumors, so registrations that keep tumor volumes will inevitably keep that change, causing errors in the metrics; for landmarks away from tumors, there will be no difference for volume-preserving and similarity-based registrations. 
%STSR offers a direct measurement of tumor changes during registration, surpassing the limitations of other common metrics like Dice and Landmark Distance. The Dice score primarily focuses on aligning the outline of the foreground, disregarding the tumor information contained within the organ. Consequently, the Dice score fails to capture the changes in tumor volume accurately. Regarding Landmark Distance, it's important to note that landmarks near the tumor area can be affected by tumor growth. Consequently, registrations that preserve tumor volumes will inherently retain these changes, leading to metric errors. Conversely, for landmarks located away from tumors, there will be no distinction between volume-preserving and similarity-based registrations.
% it is possible to have carefully selected landmarks, but takes much labors.
%Therefore, it is necessary to incorporate STSR metric into our experiments for comprehensive evaluation.

% Furthermore, we follow previous work~\cite{NichaChitphakdithai2010NonrigidRW} and conduct another evaluation to show the advantage of our methods in clinical settings. Please refer to Exp~\ref{sub:exp1}.
% In addition, we align with prior research~\cite{NichaChitphakdithai2010NonrigidRW} and incorporate an additional evaluation to highlight the superiority of our methods in clinical scenarios. For detailed information, please refer to Exp~\ref{sub:exp1}.
%}

%\textbf{Bias in STSR Metric (\Rth)}
%{Our method does not "explicitly" optimize STSR since it does not know the exact tumor and the organ segmentation, which is required to calculate STSR. Plus, the metric and the method all focus on evaluating/performing volume-preservation registration, so it is natural for our method to optimize the STSR metric. }

%\textbf{Minor Improvement in Dice (\Ro)}~\label{sub:other_metrics}
%{The Dice score inadequately captures the preservation of tumors during registration, which is a key focus of our method. Hence, it is significant for our method to achieve a comparable Dice score while outperforming others in the STSR metric, which directly measures tumor preservation.
% As above mentioned, Dice failed to show the preservation of tumors in registration, which is the main contribution of our method. Therefore, it would be good enough for our method to achieve comparable Dice score while performing best in STSR metric.

% However, it should be noted that the Dice score can only indicate how well the outline of the foreground is aligned. For the alignment of inner structure and the preservation of tumors, we should refer to Lm. Dist and STSR, respectively, and Exp~\ref{exp1} also shows a good evaluation.
% We understand that the STSR metrics might be biased towards us since our method aims to preserve tumor volumes. However, our method also  and Landmark Distance with other methods, making it the best comprehensively. Besides, STSR is also a direct metric that measures change of volume, which is important in clinical applications.
%}

\textbf{New Evaluation on GT Flow (\Ro \&\Rth)}
\label{sub:exp1}
{To complement adopted metrics, we have conducted an additional evaluation to compare our method with GT registration. We selected 5 pairs of fixed and moving brain images from test data and asked 3 expert radiographers to manually annotate dense landmarks. We use a landmark-based registration method with manual adjustment to register these images. The resulting registration, confirmed by experts, was viewed as  GT to measure RMSE between GT and predicted flows. 
% The results can be visualized in the figure, where the rightmost picture is the moving image, and the others shows differences between error maps of normal methods and our methods (red means our method has smaller errors while blue is the opposite). The blue outlines tumors warped by normal methods and the green line denotes tumors warped by our methods.
Quantitative results are shown below. On average, our method has an improvement of 0.38 in non-tumor area, 1.10 in tumor area, and 0.40 in the whole image in RMSE with GT flow. This clearly shows that our method surpasses previous works and our advantage is more obvious in tumor regions attributed to tumor volume preservation.}
 

%The quantitative and qualitative results are presented in the following: 
% \begin{figure}[ht]
% \vspace{-0.3cm}
%     \centering
%     \setlength\tabcolsep{1.6pt}
%     \begin{tabular}{cccc}
%     \includegraphics[width=.23\linewidth]{iccv2023AuthorKit/Figure/rebuttal/1.png}&
%     \includegraphics[width=.23\linewidth]{iccv2023AuthorKit/Figure/rebuttal/2.png}&
%     \includegraphics[width=.23\linewidth]{iccv2023AuthorKit/Figure/rebuttal/3.png}&
%     \includegraphics[width=.23\linewidth]{iccv2023AuthorKit/Figure/rebuttal/4.png} \\
%     Moving& VTN & VXM & TSM
%     \vspace{-0.4cm}
%     \end{tabular}
%     % \caption{Visualization on evaluation with GT flow. }
%     % \caption{Accurate registration by GT flow. Red is the landmarks in the fixed image, blue is the corresponding landmarks in moving images and green is the warped landmarks from blue points. Points not in the plane are projected.}
%     % \label{fig:exp1}
% \end{figure}
% \vspace{-0.5cm}
\newcommand{\setgray}{\cellcolor[gray]{.9}}
\begin{table}[h]
\vspace{-0.41cm}
\centering
\resizebox{.75\linewidth}{!}
{
\begin{tabular}{lccc}
\toprule[1.3pt]
\multirow{2}{*}{Method} &\multicolumn{3}{c}{$\text{RMSE (unit is pixel)}\downarrow$  in}    \\ 
\cline{2-4}
    & Organ (Non-Tumor) & Tumor & Whole Image  \\ 
    \midrule[0.7pt]
     VTN   &   7.26    & 11.28              & 7.42   \\ 
    \setgray VTN(Ours)    & \setgray 6.86     & \setgray 10.10               & \setgray 6.99  \\ 
    VXM   & 7.10 & 11.01 & 7.26 \\ 
    \setgray VXM(Ours) & \setgray 6.73 & \setgray 9.31 & \setgray 6.84     \\ 
    TSM  & 7.69 & 10.50 & 7.76 \\ 
    \setgray TSM(Ours) & \setgray 7.32 & \setgray 10.07 & \setgray 7.41   \\ 
    % LapIRN \\
    % HyperMorph \\
\bottomrule[1.3pt]
\end{tabular}
}
\vspace{-0.48cm}
\end{table}


%Our method demonstrates superior performance, particularly in tumor areas. This is attributed to our method's accurate preservation of tumor volumes, aligning with clinical requirements, whereas other methods may excessively alter tumor volumes.

\textbf{Adapt to Recent Methods (\Ro)} 
Great point! As an adaptable method, our two-stage unsupervised learning strategy can be incorporated into more advanced registration frameworks, such as LapIRN and HyperMorph. Due to limited time during rebuttal, we only tried adapting our method to LapIRN on BraTS20 (using our two-stage strategy on the third stage of LapIRN). As shown in the table, the performance is clearly improved in $|J_\theta|$ and STSR while maintained comparable on others,
% the performane is improved by ?? in DICE, ?? in landmark distances, and ??? in STSR, 
demonstrating the effectiveness and generality of our method. We will add comparisons with LapIRN and HyperMorph in the camera-ready.

%{We add additional recent works in the field and we have evaluated the performance of two recent registration methods, LapIRN~\cite{mok2020large} and HyperMorph~\cite{hoopes2021hypermorph} on our dataset. As in the following, recent advanced approaches fail to adequately preserve the volume of tumors, as indicated by the higher STSR metric  (we only display the result of one implementation to save space). 

% \newcommand{\setgray}{\cellcolor[gray]{.9}}
\begin{table}[ht]
\centering
\vspace{-0.38cm}
\resizebox{.85\linewidth}{!}
{
\begin{tabular}{lccccc}
\toprule[1.3pt]
 Method & Dice \uparrow & Lm. Dist \downarrow & $|J_\theta|<0(\%)$ \downarrow  & Std. $|J_\theta|$ \downarrow & STSR \downarrow  \\ 
    \midrule[0.7pt]      
    LapIRN & 0.975 & 3.40 & 3.020 & 0.301 & 1.889 \\ 
    \rowcolor[gray]{.9} LapIRN(Ours) & 0.974 & 3.36 & 0.040 & 0.105 & \textbf{1.224}\\
\bottomrule[1.3pt]
\end{tabular}
}
\vspace{-0.45cm}
\end{table}


==> iccv2023AuthorKit/rebuttal/others.tex <==
\textbf{"Strategy" Instead of "Framework" (\Ro)} 
{
Thanks for the suggestion. We agree with it and will revise "framework" to "strategy". }

\textbf{Missing References and Comparisons (\Rt)}
{Thanks for providing the references. We will cite and discuss them in the camera-ready. During the rebuttal, we added one more comparison to a latest work, LapIRN (please refer to the question "Adapt to Recent Methods"). We will compare to more latest works in the camera-ready.
}

\textbf{Clarity Issues(\Rt)}
{$D'(x)$ is defined in Eq.7, representing the relative volume change of voxel $x$ with respect to organ areas. 
$L_{reg}$ in Eq.13 is the smoothness regularization of the deformation field, as in VoxelMorph.
We will add an intensity bar in Fig.~3 and improve the clarity of our paper.
}

\textbf{Why Fixed Soft Tumor Mask (\Rt)}
{The soft tumor mask is estimated based on the fact that mainstream registration methods, which optimize image similarity, can vastly alter tumor volume. Thus, we do not need to train the first stage, but instead, utilize this property to estimate tumor mask. 
Also, the mask has to be fixed in the second stage, because the updated deformation field in this stage aims at registration with little volume change in tumors, and is thus unsuitable for tumor mask estimation.
% The mask has to be fixed in the second stage, as we preserve tumor volume during registration. This means the updated deformation field without volume changes in this stage is unsuitable for tumor mask estimation.
}

\textbf{Issues in Equations (\Rth)}
{Thanks for bringing them to our attention. We will revise them accordingly.}

==> iccv2023AuthorKit/rebuttal/reviewer1.tex <==
\textbf{Clarify Technical Novelty} 
{Thanks for pointing it out. We agree that "strategy" is a more suitable term for our proposed method, and we will make the necessary changes to our paper. }

\textbf{Compare with Recent Works} 
{Thanks for your suggestion! It would indeed add more efficacy to our proposed strategy to experiment with recent works in the field. Therefore, we have tested the performance of LapIRN~\cite{mok2020large} and HyperMorph~\cite{hoopes2021hypermorph} on our data, which is shown in Table~\ref{tab:rtab1}.

% results not come out yet
According to the table, recent advanced works failed to preserve the volume of tumors (higher STSR) compared to our proposed method (We only display the result of one implementation of our methods to save space). }
\newcommand{\setgray}{\cellcolor[gray]{.9}}
\begin{table}[hb]
\centering
\resizebox{1.\linewidth}{!}
{
\begin{tabular}{lccccc}
\specialrule{.8pt}{0pt}{2pt}
\multirow{2}{*}{Methods} & \multicolumn{5}{c}{LiTs17}    \\ 
\cline{2-6} 
    & Dice \uparrow & Lm. Dist \downarrow & $|J_\theta|<0(\%)$ \downarrow  & Std. $|J_\theta|$ \downarrow & STSR \downarrow  \\ 
    \specialrule{.4pt}{2pt}{0pt}
    \setgray VTN(Ours)   & \setgray0.908  & \setgray10.77    & \setgray2.956               & \setgray1.124             & \setgray\textbf{1.260} \\
        LapIRN \\
    HyperMorph \\
\specialrule{.4pt}{2pt}{0pt}
\specialrule{.8pt}{0pt}{2pt}
\multirow{2}{*}{Methods} &\multicolumn{5}{c}{BraTS20}    \\ 
\cline{2-6}
    & Dice \uparrow & Lm. Dist \downarrow & $|J_\theta|<0(\%)$ \downarrow  & Std. $|J_\theta|$ \downarrow & STSR \downarrow  \\ 
    \specialrule{.4pt}{2pt}{0pt}
    \setgray VTN(Ours)   & \setgray0.9738 & \setgray3.10     & \setgray0.596               & \setgray0.285             & \setgray\textbf{1.416}\\ 
    LapIRN \\
    HyperMorph \\
\specialrule{.8pt}{0pt}{2pt}
\end{tabular}
}
\caption{Comparison with recent advanced works.}
\label{tab:rtab1}
\end{table}
\vspace{-0.25cm}

\textbf{Minor Improvement in Dice} 
{Thanks for pointing it out. Indeed, the Dice has limited improvement using our methods. However, it should be noted that the Dice score can only indicate how well the outline of the foreground is aligned. For the alignment of inner structure and the preservation of tumors, we should refer to Lm. Dist and STSR, respectively.
}

\textbf{Validity of Metrics STSR and TSR}
{We understand that STSR is not a wide-accepted metric yet, since preserving tumor volumes is an undermined topic with relatively few recent works. Therefore, we conduct another experiment to evaluate our method on cases with manually registered images, following~\cite{NichaChitphakdithai2010NonrigidRW}. To be specific, we pick 5 fix-moving image pairs from our brain test data and ask an expertise in radiography to 
% annotate dense landmarks over the images. We then use optimization method to register images based on the annotated landmark error within fixed and moving images. 
manually annotate dense landmarks and register these images to meet the desired clinical requirements. We then use the manual registration flow as GT flow to measure the accuracy of registration methods.

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\linewidth,height=0.4\linewidth]{Copy.png}
\caption{Accurate registration by GT flow}
\label{fig:gt_lmk}
\end{figure}

\begin{table}[h]
\centering
\resizebox{1.\linewidth}{!}
{
\begin{tabular}{lcccc}
\specialrule{.8pt}{0pt}{2pt}
\multirow{2}{*}{Methods} &\multicolumn{4}{c}{$MSE\downarrow$ in}    \\ 
\cline{2-5}
    & Tumor core & Tumor & Organ & Whole image  \\ 
    \specialrule{.4pt}{2pt}{0pt}
     VTN   & 0.9738 & 3.10     & 0.596               & 0.285   \\ 
    \setgray VTN(Ours)   & \setgray0.9738 & \setgray3.10     & \setgray0.596               & \setgray0.285   \\ 
    VXM   & 0.9738 & 3.10     & 0.596               & 0.285   \\ 
    \setgray VXM(Ours)   & \setgray0.9738 & \setgray3.10     & \setgray0.596               & \setgray0.285   \\ 
    TSM  & 0.9738 & 3.10     & 0.596               & 0.285   \\ 
    \setgray TSM(Ours)   & \setgray0.9738 & \setgray3.10     & \setgray0.596               & \setgray0.285   \\ 
    LapIRN \\
    HyperMorph \\
\specialrule{.8pt}{0pt}{2pt}
\end{tabular}
}
\caption{Evaluation on GT flow.}
\label{tab:rtab2}
\end{table}

According to Fig.~\ref{fig:gt_lmk}, the GT flow accurately register the landmarks. The results is shown in Table~\ref{tab:rtab2}. The $MSE$ is the mean square error between GT flow and predicted flow. Our method has better performance on near-tumor areas since our method correctly preserves the tumor volume as clinical situation requires while other methods may excessively change the tumor volumes.
}


==> iccv2023AuthorKit/rebuttal/reviewer2.tex <==
\textbf{Lack of Relevant References}
{
Thanks for provding the references! We will add them in our paper.
}

\textbf{Issues with Readability and Clarity}
{
Thanks for pointing it out. The missing explanation will be added.
}

\textbf{Unclear Usage of Soft Tumor Mask}
{
The soft mask serves as a good indicator for potential tumor areas in stage two while the deformation field in the final output is trying to optimize the preservation of tumors based on the "soft mask" indicators. Therefore, the soft mask can be unchanged in stage two and from the experiment, we find that it suffices to provide good guidance. However, it may also be possible to use dynamic tumor mask, which is an interesting future topic.
}

==> iccv2023AuthorKit/rebuttal/reviewer3.tex <==
\textbf{Issues in Equations}
{Thanks for pointing it out. We will fix it in our paper.}

\textbf{Bias in STSR Metric}
{
We understand that the STSR metrics might be biased towards us since our method aims to preserve tumor volumes. However, our method also achieve comparable Dice and Lm. Dist with other methods, making it the best comprehensively. Besides, STSR is also a direct metric that measures change of volume, which is important in clinical applications.

Furthermore, to demonstrate the advantage of our method in practice, we conduct another evaluation, following~\cite{NichaChitphakdithai2010NonrigidRW}, based on the manual registration of experts in the field. The details could refer to Table~\ref{tab:rtab2} and the 4th subsection in Section~\ref{s1}. 
}

